Asynchronous Muddy Children Puzzle (work in progress)

In this work-in-progress paper we explore using the recently introduced VLSM formalism to define and reason about the dynamics of agent-based systems. To this aim we use VLSMs to formally present several possible approaches to modeling the interactions in the Muddy Children Puzzle as protocols that reach consensus asynchronously.

==> eptcsdata.tex <==
\providecommand{\firstpage}{152}
\providecommand{\publicationstatus}{H. Cheval, L. Leu\c{s}tean, A. Sipo\c{s} (Eds.):\\ 7th Symposium on Working Formal Methods (FROM 2023)\\
EPTCS 389, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.389.13}{10.4204/EPTCS.389.13}}

